Grassmannian Learning: Embedding Geometry Awareness in Shallow and Deep Learning

Modern machine learning algorithms have been adopted in a range of signal-processing applications spanning computer vision, natural language processing, and artificial intelligence. Many relevant problems involve subspace-structured features, orthogonality constrained or low-rank constrained objective functions, or subspace distances. These mathematical characteristics are expressed naturally using the Grassmann manifold. Unfortunately, this fact is not yet explored in many traditional learning algorithms. In the last few years, there have been growing interests in studying Grassmann manifold to tackle new learning problems. Such attempts have been reassured by substantial performance improvements in both classic learning and learning using deep neural networks. We term the former as shallow and the latter deep Grassmannian learning. The aim of this paper is to introduce the emerging area of Grassmannian learning by surveying common mathematical problems and primary solution approaches, and overviewing various applications. We hope to inspire practitioners in different fields to adopt the powerful tool of Grassmannian learning in their research.

==> 01_R2_plane.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file '01_R2_plane.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{574.33600191bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.79590728)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{01_R2_plane.pdf}}%
    \put(0.52317983,0.35619388){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{$O$}}}%
    \put(0.81243009,0.35997657){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x$}}}%
    \put(0.4208483,0.76024789){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$y$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{01_R2_plane.pdf}}%
    \put(0.19785456,0.35674993){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{\textbf{\textit{$\st{2}{1}$}}}}}%
    \put(0.67394348,0.20520629){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{\textbf{\textit{$\st{2}{1}$}}}}}%
    \put(0.59466154,0.69226557){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{\textbf{\textit{$\grass{2}{1}$}}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{01_R2_plane.pdf}}%
    \put(0.6256127,0.36389116){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{\textbf{\textit{$1$}}}}}%
    \put(0.457134,0.56845003){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{\textbf{\textit{$1$}}}}}%
    \put(0.642726,0.50514225){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\textbf{\textit{$\grass{2}{1}$ generators.}}}}}%
  \end{picture}%
\endgroup%


==> 01_R3_gr.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file '01_R3_gr.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{430.80882018bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.61765095)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{01_R3_gr.pdf}}%
    \put(0.33362902,0.37113738){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{$\u_i$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{01_R3_gr.pdf}}%
    \put(0.65725726,0.39437656){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\v_i$}}}%
    \put(0.78993455,0.44557171){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal{V}$}}}%
    \put(0.49543348,0.20993986){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\theta_i$}}}%
    \put(0.21143914,0.46886309){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{$\mathcal{U}$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{01_R3_gr.pdf}}%
  \end{picture}%
\endgroup%


==> gda.svg.2018_06_04_08_50_33.0.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'gda.svg.2018_06_04_08_50_33.0.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{413.94768963bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.31471026)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{gda.svg.2018_06_04_08_50_33.0.pdf}}%
    \put(0.54527365,0.08590219){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.13821278\unitlength}\raggedright $\mathcal{H}$\end{minipage}}}%
    \put(0.77931703,0.03725573){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.0581911\unitlength}\raggedleft $\balpha$\end{minipage}}}%
    \put(0.0590833,0.12449695){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.13504755\unitlength}\centering $\mathcal{M}$\end{minipage}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{gda.svg.2018_06_04_08_50_33.0.pdf}}%
  \end{picture}%
\endgroup%


==> grass_op_paradigm_horizontal.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'grass_op_paradigm_horizontal.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{1101.82857216bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.06845763)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{grass_op_paradigm_horizontal.pdf}}%
    \put(0.01537714,0.04327533){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.15034747\unitlength}\centering Training Data\end{minipage}}}%
    \put(0.32680801,0.04327533){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.09692978\unitlength}\centering Grassmannian Representation\end{minipage}}}%
    \put(0.60631678,0.04327574){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.10424233\unitlength}\centering Kernelized Learning Algorithm\end{minipage}}}%
    \put(0.85968766,0.04327534){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.09952286\unitlength}\centering Lower Dimensional Representation\end{minipage}}}%
  \end{picture}%
\endgroup%


==> grassmimo_ii.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'grassmimo_ii.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{494.65341441bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.72902585)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{grassmimo_ii.pdf}}%
    \put(0.93468021,0.3442526){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{Grassmannian $\mathcal{M}$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{grassmimo_ii.pdf}}%
    \put(0.16565095,0){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{ }}}%
    \put(0.06399246,0.30035459){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.49442991\unitlength}\raggedright {\small Multi-user channel trajectory with mixed mobility}\end{minipage}}}%
    \put(0.24189479,0.6700218){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.56836331\unitlength}\raggedright {\small Channel trajectory for slow mobility user}\end{minipage}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{grassmimo_ii.pdf}}%
    \put(0.47986809,0.69769808){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.06238136\unitlength}\raggedright  \end{minipage}}}%
  \end{picture}%
\endgroup%


==> lrr.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'lrr.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{577.51739542bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.60403704)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{lrr.pdf}}%
    \put(0.4123938,0.06184429){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.11622143\unitlength}\raggedright $\U$\end{minipage}}}%
    \put(0.39639047,0.43142087){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.53505276\unitlength}\raggedright {$\x_1 = \tp{\begin{bmatrix} 1 & 0 & 1 \end{bmatrix}}$}\end{minipage}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{lrr.pdf}}%
    \put(0.01067781,0.45123158){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.11622143\unitlength}\raggedright $\B_1$\end{minipage}}}%
    \put(0.05092047,0.16516137){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.17871062\unitlength}\raggedright $\e_1$\end{minipage}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{lrr.pdf}}%
    \put(0.37290815,0.21801841){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.17871062\unitlength}\raggedright $\theta_1$\end{minipage}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{lrr.pdf}}%
  \end{picture}%
\endgroup%


==> rec.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'rec.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{420.86425781bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.52417946)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{rec.pdf}}%
    \put(0.44307542,0.0091678){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textit{[Not supported by viewer]}}}}%
    \put(0.54108802,0.0091678){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textit{[Not supported by viewer]}}}}%
    \put(0.73889527,0.0091678){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textit{[Not supported by viewer]}}}}%
    \put(0.64444676,0.06441126){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.31655007,0.28182103){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.24170408,0.45824371){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textit{[Not supported by viewer]}}}}%
    \put(0.24170408,0.37092339){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textit{[Not supported by viewer]}}}}%
    \put(0.24170408,0.19806481){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textit{[Not supported by viewer]}}}}%
    \put(0.73889527,0.19806481){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.54465212,0.45824371){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.44307542,0.45824371){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.44307542,0.19806481){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.44307542,0.35666701){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.44307542,0.28182103){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.54465212,0.35666701){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.54465212,0.19806481){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.73889527,0.35666701){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.73889527,0.45824371){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.73889527,0.28182103){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.54465212,0.28182103){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.63731858,0.46358985){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
    \put(0.64444676,0.19806481){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{\textbf{[Not supported by viewer]}}}}%
  \end{picture}%
\endgroup%


==> ssc_exp.tex <==
\FloatBox*[\linewidth]{
    \begin{example}[SSC on three-ring data] \label{ex:ssc} \normalfont
    %\includegraphics[page=1,width=\linewidth]{grass_kernel}
        %\resizebox{0.6\textwidth}{!}{%
        %\def\svgwidth{\linewidth}
        %\input{figs/grass_op_paradigm.pdf_tex}}
	We consider $N=1550$ two-dimensional three-ring data with $k=3$ clusters.
	We use the steepest
	descent on $\grass{N}{k}$ with the penalty $\beta=0.01$ and
	varying $\sigma\in \{0.1,1,1.6,3,5\}$, the bandwidth in Gaussian kernel used for
	constructing the affinity $\W$. Each column corresponds to
	a $\sigma$ with the heat map of $\U\tp{\U}$, the embedding of $\U$ in $\sR^3$,
	and the clustering results displayed. The structural information can be infer  from the heat map. For example, for  $\sigma=1.6$, one can observe  three  diagonal blocks (including a tiny one in white) in the
	heat map, indicating the existence of  three clusters. We note that the value of  $\sigma$ has a signifcant effect on  the quality of clustering, governing how the Grassmannian optimization can disentangle data in the low-dimensional latent space determined by $\U$. For small  $\sigma$, the similarity measures between data samples are reduced. As a result, data samples are pushed away from each other and appear  isolated. On the other hand, increasing  $\sigma$ tends to amplify
similarity and thereby pulls  data samples  together, resulting in parallel circles on the sphere in the latent space. As can be observed from Fig.~\ref{fig:ex:ssc}, both the cases of $\sigma$ being  too large or too small all lead to undesirable clustering results, suggesting the need of optimizing the parameter. 
With a properly chosen $\sigma$ ($1.6$ in this case), all three clusters are  concentrated in separate  small regions in the latent space generated by $\U$ (see the second row of Fig.~\ref{fig:ex:ssc}). Consequently, the three data rings are correctly clustered as marked in different colours (see the bottom  row of Fig.~\ref{fig:ex:ssc}). \\ 
	\begin{subfigure}[t]{0.03\textwidth}
		\vskip -8.5cm
		\rotatebox{90}{$\U\tp{\U}$}
		\vskip 2.2cm
		\rotatebox{90}{$\U$}
		\vskip 2cm
		\rotatebox{90}{Clustering}
	\end{subfigure}%
	\begin{subfigure}[t]{0.97\textwidth}
	\begin{center}
	\includegraphics[width=\textwidth]{figs/ssc_bk-eps-converted-to.pdf}
	\end{center}
    \end{subfigure}
    \caption{Example of sparse spectral clustering via Grassmann optimization.} \label{fig:ex:ssc}
    %\caption{Illustration of the Example. \textbf{Left:    } The objective of the original formulation \eqref{eq:mcp}
	%using Frobenius norm. \textbf{Right:    } The objective alternatively formulated using chordal distance.}
    \end{example}
} %FloatBox

